A high-order, fully well-balanced, unconditionally positivity-preserving finite volume framework for flood simulations

In this work, we present a high-order finite volume framework for the numerical simulation of shallow water flows. The method is designed to accurately capture complex dynamics inherent in shallow water systems, particularly suited for applications such as tsunami simulations. The arbitrarily high-order framework ensures precise representation of flow behaviors, crucial for simulating phenomena characterized by rapid changes and fine-scale features. Thanks to an {\it ad-hoc} reformulation in terms of production-destruction terms, the time integration ensures positivity preservation without any time-step restrictions, a vital attribute for physical consistency, especially in scenarios where negative water depth reconstructions could lead to unrealistic results. In order to introduce the preservation of general steady equilibria dictated by the underlying balance law, the high-order reconstruction and numerical flux are blended in a convex fashion with a well-balanced approximation, which is able to provide exact preservation of both static and moving equilibria. Through numerical experiments, we demonstrate the effectiveness and robustness of the proposed approach in capturing the intricate dynamics of shallow water flows, while preserving key physical properties essential for flood simulations.

==> Abstract.tex <==



In this work, we present a high-order finite volume framework for the numerical simulation of shallow water flows.
The method is designed to accurately capture complex dynamics inherent in shallow water systems, particularly suited for applications such as tsunami simulations. 
The arbitrarily high-order framework ensures precise representation of flow behaviors, 
crucial for simulating phenomena characterized by rapid changes and fine-scale features. 
Thanks to an {\it ad-hoc} reformulation in terms of production-destruction terms, 
the time integration ensures positivity preservation without any time-step restrictions, 
a vital attribute for physical consistency, especially in scenarios where negative water depth 
reconstructions could lead to unrealistic results. 
In order to introduce the preservation of general steady equilibria dictated by the underlying balance law, 
the high-order reconstruction and numerical flux are blended in a convex fashion with a well-balanced approximation, 
which is able to provide exact preservation of both static and moving equilibria.
Through numerical experiments, we demonstrate the effectiveness and robustness of the proposed approach in capturing 
the intricate dynamics of shallow water flows, while preserving key physical properties essential for flood simulations.

%% In this paper, we present a new arbitrary high order and structure--preserving method for the numerical solution of the Shallow Water (SW) equations. 
%% %
%% The method is obtained by coupling two general strategies: the modified Patankar Deferred Correction (mPDeC) positivity--preserving time integration scheme and a well--balanced (WB) Finite Volume (FV) spatial semidiscretization able to exactly preserve generic steady equilibria.
%% %
%% The accuracy and the structure--preserving features of the novel approach are validated on several benchmarks, including real applications.


==> Implementation.tex <==
\subsubsection{Implementation of mPDeC on WENO Scheme}\label{se_implemenation}

In the following part, we will describe how the semi-discretization, using the WENO approach, can be written and interpreted as a PDS in order to apply the mPDeC scheme. 
We will see that only small modifications in the WENO code are necessary. 
Furthermore, this interpretation is not only restricted to the WENO procedure but can also applied to other high-order FV/FD discretizations. 
Our WENO approach is working only as a generic example. Finally, the complete algorithm will be presented.

%\subsection{WENO and production-destruction systems}
%\cite-> Ghost cells -> Using the approach by Russo (checking without ghost cells-> other work)
%
First of all we must underline the fact that in order to preserve the positivity of the water height $h$, 
the mPDeC scheme is going to be applied only to the first equation of system~\eqref{eq:CL} as $h$ is the only variable that must stay nonnegative.
Thus, a simple DeC approach is going to be used to evolve the momentum equations.
So from now on, we shall only talk about the modifications introduced for the first equation to turn it into a production-destruction system.
Given the foundations of finite volume schemes, each control volume has fluxes entering and exiting its boundary and, for each boundary
face, the flux going from element $\alpha=[i,j]$ to element $\beta=[l,r]$ is going to be equal in module and opposite in sign to the flux from element $\beta$ to element $\alpha$. This is the key feature for turning a finite volume schemes into a PDS. Note that the source is zero on $h$ component.\\
Therefore, we can define the production and destruction terms for a general $\alpha=[i,j]$ and the neighboring $\beta=[l,r]$ as 
\begin{equation}\label{eq:PDSforWENO}
	\begin{split}
		p_{[i,j],[i-1,j]}({\bU})= +\frac{1}{\Delta x}\overline{\bF}_{i-1/2,j} (\bU)^+, \quad d_{[i,j],[i-1,j]}({\bU})=- \frac{1}{\Delta x}\overline{\bF}_{i-1/2,j} (\bU)^-,\\
		p_{[i,j],[i+1,j]}({\bU})= -\frac{1}{\Delta x}\overline{\bF}_{\iip,j} (\bU)^-, \quad d_{[i,j],[i+1,j]}({\bU})=+ \frac{1}{\Delta x}\overline{\bF}_{\iip,j} (\bU)^+,\\
		p_{[i,j],[i,j-1]}({\bU})= + \frac{1}{\Delta y}\overline{\bG}_{i,j-1/2} (\bU)^+, \quad d_{[i,j],[i,j-1]}({\bU})=-\frac{1}{\Delta y} \overline{\bG}_{i,j-1/2} (\bU)^-,\\
		p_{[i,j],[i,j+1]}({\bU})= - \frac{1}{\Delta y} \overline{\bG}_{i,j+1/2} (\bU)^-, \quad d_{[i,j],[i,j+1]}({\bU})=+ \frac{1}{\Delta y}\overline{\bG}_{i,j+1/2} (\bU)^+,
	\end{split}
\end{equation}
where with the superscript $\,^+$ and $\,^-$ we denote the positive and the negative part respectively. All the other $p_{\alpha,\beta}$ and $d_{\alpha,\beta}$ not defined here are set to 0. Clearly, this define a conservative and positive PDS, as the properties in Definition \ref{def:POSCONSPDS} are verified. The visualization of the production and destruction terms in Figure~\ref{fig:omega_ij} may help the reader.
We clearly observe that the matrices $(p_{\alpha,\beta})$ and $(d_{\alpha,\beta})$ are $S\times S$ sparse matrices, with, at most, 4 nonzero entries per row and $S=N_x\cdot  N_y$.


%the first step to build the algorithm is defining the production and destruction terms, $p_{ij}$ and $d_{ij}$,
%which are going to have a sparse matrix shape. 
%These are $S\times S$ matrices, where $S=N_x\times N_y$ is the total number of control volumes
%used to discretize the computational domain $\Omega$. 
%Although $p_{ij}$ and $d_{ij}$ are as big as the total number of elements, 
%each row belonging to element $i$ is made up by all zeroes except for those four locations corresponding to the production 
%and destruction terms given by the numerical flux computed at its four boundaries (see Fig.~\ref{fig:omega_ij}).
%Few precautions has to be taken in order to always have $p_{ij},d_{ij}>0$.
%
\begin{figure}
\centering
\scalebox{1.3}{
\begin{tikzpicture}
%
%\draw [-stealth] (0,0) -- (5.5,0);
%\node [black,scale=1] at (5.5,-0.5) {$x$};
%
%\draw [-stealth] (0,0) -- (0,5.5);
%\node [black,scale=1] at (-0.5,5.5) {$y$};

\draw (0.,2) -- (2,2) -- (2,3.5) -- (0.,3.5) -- (0.,2);
\draw (2,2) -- (3.5,2) -- (3.5,3.5) -- (2,3.5) -- (2,2);
\draw (3.5,2) -- (5.5,2) -- (5.5,3.5) -- (3.5,3.5) -- (3.5,2);
\draw (2,0.5) -- (3.5,0.5) -- (3.5,2) -- (2,2) -- (2,0.5);
\draw (2,3.5) -- (3.5,3.5) -- (3.5,5) -- (2,5) -- (2,3.5);

\node [black,scale=0.8] at (0.9,2.75) {$\Omega_{i-1,j}$};
\node [black,scale=0.8] at (2.75,2.75) {$\Omega_{i,j}$};
\node [black,scale=0.8] at (4.6,2.75) {$\Omega_{i+1,j}$};
\node [black,scale=0.8] at (2.75,4.25) {$\Omega_{i,j+1}$};
\node [black,scale=0.8] at (2.75,1.25) {$\Omega_{i,j-1}$};

\node [red, scale=0.7, anchor=south] at (1.9,2.7) {$\overline{\bF}_{i-1/2,j}(\bU)$};
%\node [red, scale=0.7, anchor=south] at (1.9,2.48) {$d_{[i,j],[i-1,j]}$};

\draw [-stealth,red] (1.55,2.7) -- (2.25,2.7);
%\draw [stealth-,red] (1.55,2.8) -- (2.25,2.8);


%\node [red, scale=0.7, anchor=base] at (3.6,2.48) {$p_{[i,j],[i+1,j]}$};
\node [red, scale=0.7, anchor=south] at (3.6,2.7) {$\overline{\bF}_{i+1/2,j}(\bU)$};

\draw [stealth-,red] (3.95,2.7) -- (3.25,2.7);
%\draw [stealth-,red] (3.95,2.8) -- (3.25,2.8);


%\node [red, scale=0.7, anchor=base east] at (2.65,1.75) {$p_{[i,j],[i,j-1]}$};
\node [red, scale=0.7, anchor=base west] at (2.85,2.05) {$\overline{\bG}_{i,j-1/2}(\bU)$};

\draw [-stealth,red] (2.75,1.65) -- (2.75,2.35);
%\draw [stealth-,red] (2.8,1.65) -- (2.8,2.35);


%\node [red, scale=0.7, anchor=base east] at (2.65,3.7) {$d_{[i,j],[i,j+1]}$};
\node [red, scale=0.7, anchor=base west] at (2.85,3.65) {$\overline{\bG}_{i,j+1/2}(\bU)$};

\draw [-stealth,red] (2.75,3.15) -- (2.75,3.85);
%\draw [stealth-,red] (2.8,3.15) -- (2.8,3.85);

\end{tikzpicture}}\hfill
\scalebox{1.3}{
	\begin{tikzpicture}
		%
		%\draw [-stealth] (0,0) -- (5.5,0);
		%\node [black,scale=1] at (5.5,-0.5) {$x$};
		%
		%\draw [-stealth] (0,0) -- (0,5.5);
		%\node [black,scale=1] at (-0.5,5.5) {$y$};
		
		\draw (0.,2) -- (2,2) -- (2,3.5) -- (0.0,3.5) -- (0.,2);
		\draw (2,2) -- (3.5,2) -- (3.5,3.5) -- (2,3.5) -- (2,2);
		\draw (3.5,2) -- (5.5,2) -- (5.5,3.5) -- (3.5,3.5) -- (3.5,2);
		\draw (2,0.5) -- (3.5,0.5) -- (3.5,2) -- (2,2) -- (2,0.5);
		\draw (2,3.5) -- (3.5,3.5) -- (3.5,5) -- (2,5) -- (2,3.5);
		
		\node [black,scale=0.8] at (0.9,2.75) {$\Omega_{i-1,j}$};
		\node [black,scale=0.8] at (2.75,2.75) {$\Omega_{i,j}$};
		\node [black,scale=0.8] at (4.6,2.75) {$\Omega_{i+1,j}$};
		\node [black,scale=0.8] at (2.75,4.25) {$\Omega_{i,j+1}$};
		\node [black,scale=0.8] at (2.75,1.25) {$\Omega_{i,j-1}$};
		
		\node [red, scale=0.7, anchor=base] at (1.9,2.48) {$p_{[i,j],[i-1,j]}$};
		\node [red, scale=0.7, anchor=south] at (1.9,2.82) {$d_{[i,j],[i-1,j]}$};
		
		\draw [-stealth,red] (1.55,2.7) -- (2.25,2.7);
		\draw [stealth-,red] (1.55,2.8) -- (2.25,2.8);
		
		
		\node [red, scale=0.7, anchor=base] at (3.6,2.48) {$p_{[i,j],[i+1,j]}$};
		\node [red, scale=0.7, anchor=south] at (3.6,2.82) {$d_{[i,j],[i+1,j]}$};
		
		\draw [-stealth,red] (3.95,2.7) -- (3.25,2.7);
		\draw [stealth-,red] (3.95,2.8) -- (3.25,2.8);
		
		
		\node [red, scale=0.7, anchor=base east] at (2.65,1.75) {$p_{[i,j],[i,j-1]}$};
		\node [red, scale=0.7, anchor=base west] at (2.85,1.75) {$d_{[i,j],[i,j-1]}$};
		
		\draw [-stealth,red] (2.7,1.65) -- (2.7,2.35);
		\draw [stealth-,red] (2.8,1.65) -- (2.8,2.35);
		
		
		\node [red, scale=0.7, anchor=base east] at (2.65,3.7) {$d_{[i,j],[i,j+1]}$};
		\node [red, scale=0.7, anchor=base west] at (2.85,3.7) {$p_{[i,j],[i,j+1]}$};
		
		\draw [-stealth,red] (2.7,3.15) -- (2.7,3.85);
		\draw [stealth-,red] (2.8,3.15) -- (2.8,3.85);
		
\end{tikzpicture}}
\caption{Cell $\Omega_{i,j}$, its four neighbors and its production and destruction terms.}\label{fig:omega_ij}
\end{figure}
%
Once the production and destruction matrices have been assembled, the next step consist in running the mPDeC algorithm in Eq.~\eqref{eq:explicit_dec_correction}. Note that the matrix built in \eqref{eq:matrixMPDeC} is sparse as well with at most 5 nonzero entries for each row (4 nonzero entries of the production/destruction terms and the diagonal term).
Hence, in the numerical computations we will use the classical Jacobi iterative method, see Algorithm \ref{algo:jacobi}, to obtain the solution of system \eqref{eq:explicit_dec_correction} at each iteration. 
Indeed, it is provable \cite{offner2020arbitrary,burchard2003high} that the Jacobi iteration algorithm converges when applied on the matrix defined in \eqref{eq:matrixMPDeC}. 

In all calculations, we set the tolerance to machine precision and the algorithm converge towards the solution in few iterations. Experimentally, we have seen that usually 10-20 iterations suffice, in the worst cases 40 iterations are needed and the number of iterations do not depend much on the mesh size. 
Overall, considering the assembly the mass matrix, the inversion of the system with Jacobi iterations, the whole mPDeC procedure increases the computational costs of around 18\% with respect to the original DeC algorithm using the same CFL. The code has not been construct with the goal of optimizing all the procedures, so it might well be that this extra computational cost can be decreased with better implementations. The greatest advantage is anyway that no CFL restrictions are required in order to guarantee the positivity of the solution. So, a CFL$=1$ suffices to guarantee the stability of the method.
In the numerical test section, we will also detail the number of Jacobi iterations and the overhead computational cost that the method brings into the system with respect to the explicit method.


==> PrimitiveVarRecon.tex <==
\section{Reconstruction of the primitive variable}\label{sec:PrimitiveVarRecon}

The goal of this section is that of deepening the procedure to compute the coeffiecients of the polynomials and linear weights needed to compute the WENO procedure in Section \ref{sec_Space}. The results and the actual coefficients for WENO5 with 4 Gaussian quadrature points are written in Section~\ref{sec:WENO5GP4}. 

In the following assemble the system that allow to find the coefficients for the WENO polynomial at any quadrature point. The symbolic Matlab script coded for this purpose is also available 
at~\cite{ourrepo}. With few adjustments, the script can be used to compute all the ingredients needed for a 
WENO reconstruction of arbitrary high order with arbitrary high order quadrature formulae.\\
The reconstruction of the primitive variables is needed in a high order finite volume method, as  only cell averages are available from the previous time step. For the sake of simplicity we are going to 
work in a simpler one-dimensional scalar framework since the reconstruction is done dimension-by-dimension.
We consider a scalar function $u(x)$ whose cell averages $u_i$ are known. We aim at reconstructing this variable as a polynomial $v(x)$, where the polynomial may vary in different points. In particular, it will be useful to use a primitive of $v(x)$ which we denote by $\mathcal{P}(x)=\int_{x_0}^x v(s) \diff{s}$. Indeed, we can impose that for every cell average, we have
%
\begin{equation}\label{eq:sys_coeffWENO_cellave}
u_{i}=\frac{1}{\Delta x}\int_{\xin}^{\xip} u(x)\;\diff{x} \stackrel{!}{=} \int_{\xin}^{\xip} v(x) \diff{x} =\frac{\mathcal{P}(x_{\iip} )- \mathcal{P}(x_{\iin})}{\Delta x}.
\end{equation}
%
The stencil considered for this example is the one used for the WENO5 reconstruction, which is made up by five cell averages
as denoted in Figure~\ref{Fig:Space_Stencil}.
%
\begin{figure}[ht]
        \centering
\begin{tikzpicture}
\draw [thick]   (0,0) -- (10,0) node[below=2mm] {}; 
% nodes
\fill[black]    (0,0) circle (1mm) node[below=2mm] {$x_{i-5/2}$}
                (2,0) circle (1mm) node[below=2mm] {$x_{i-3/2}$}
                (4,0) circle (1mm) node[below=2mm] {$x_{i-1/2}$}
                (6,0) circle (1mm) node[below=2mm] {$x_{i+1/2}$} 
                (8,0) circle (1mm) node[below=2mm] {$x_{i+3/2}$}
                (10,0) circle(1mm) node[below=2mm] {$x_{i+5/2}$};
\node at (1,0.5) {$u_{i-2}$};
\node at (3,0.5) {$u_{i-1}$};
\node at (5,0.5) {$u_{i}$};
\node at (7,0.5) {$u_{i+1}$};
\node at (9,0.5) {$u_{i+2}$};
\end{tikzpicture} \caption{Stencil of five cell averages for WENO5 reconstruction.}\label{Fig:Space_Stencil}
\end{figure}

The next step consists in using interpolating polynomials $\varphi_{j-1/2}$, e.g.\ Lagrange polynomials at cell interfaces, to approximate the primitive $\mathcal{P}(x)$, i.e.,
%
\begin{equation}\label{eq:lagrange}
\mathcal{P}(x) = \sum_{j=k_1}^{k_2+1} a_{j-1/2}\,\varphi_{j-1/2}(x) \qquad \text{where}\qquad \varphi_{j-1/2}(x) = \prod_{\ell=k_1, i \neq j}^{k_2+1} \frac{x-x_{\ell-1/2}}{x_{j-1/2}-x_{\ell-1/2}}
\end{equation}
%
where $k_1$ and $k_2$ are the extreme indexes of the considered stencil. So, given then $k_2-k_1+1$ cell averages, the degree of the polynomial $\mathcal{P}$ will be $k_2-k_1+2$.
For instance, when working with WENO5, the reconstruction is composed by a linear combination of three lower order polynomials of degree 3, so with $\mathcal{P} \in \mathbb P_4$, obtained through three cell averages. Then, the 3 polynomials, which then depend on the whole 5 cells stencil, will be be combined with weights which depends on the quadrature points into a fifth order accurate reconstruction. 
In order to have this result, we need to compute the aforementioned three lower order polynomials and a high order polynomial made up
by information coming from the whole stencil.\\
Let us begin with the procedure to compute the high order polynomial with all available cell averages, i.e., $k_1=-2$ and $k_2=2$.
The lower order polynomials can be easily computed following the same approach explained hereafter.
In this case $\mathcal{P}(x)$ is a sixth order polynomial and $v(x)=\mathcal{P}'(x)$ is a fifth order polynomial which gives the right accuracy order. 
Using \eqref{eq:sys_coeffWENO_cellave} for all cell averages in the stencil with the definition of $\mathcal{P}$ given in \eqref{eq:lagrange} and using the property of Lagrangian polynomials $\varphi_{j-1/2}(x_{\ell -1/2}) = \delta_{j,\ell}$, we obtain a system of equations for the coefficients $a_{j-1/2}$ 
with solution
%
\begin{equation}
a_{j-1/2} = \begin{cases}
 0,  & \text{if }j=k_1, \\ 
 \sum_{\ell=-k_1}^{-k_1+j-1} u_{i+\ell}, & j=k_1+1,\dots, k_2+1. 
\end{cases}
\end{equation}
%
Finally, the expression for the high order, $ho$, approximation polynomial $v^{ho}(x)$ can be written as 
%
\begin{equation}
v^{ho}(x)= \sum_{j=k_1}^{k_2+1} a_{j-1/2}\varphi'_{j-1/2}(x) = \sum_{\ell=-k_1}^{k_2} c^{ho}_{\ell}(x) \,u_{i+\ell}= \sum_{\ell=-2}^{2} c^{ho}_{\ell}(x) \,u_{i+\ell},
\end{equation}
%
where $c^{ho}_\ell$ are obtained collecting all the coefficients and basis functions related to $u_{i+\ell}$. In this way, for any quadrature point $\tilde\xi \in [x_{i-1/2},x_{i+1/2}]$ we can evaluate this high order polynomial $v^{ho}(\tilde \xi)$.
%
Following the same procedure for three lower order polynomials, $lo$, associated to the 3-cells stencils
$S^0=\{u_{i},u_{i+1},u_{i+2}\}$, $S^1=\{u_{i-1},u_{i},u_{i+1}\}$ and $S^2=\{u_{i-2},u_{i-1},u_{i}\}$,  we obtain an expression for these low order polynomials
%
\begin{equation}
v^{lo}_j(x) = \sum_{\ell=-j}^{2-j} c^{lo}_{j\ell}(x) \,u_{i+\ell}.
\end{equation}
%
The last step concerns the computation of the ideal linear weights. These are the weights that allow to recover the high order reconstruction
from a linear combination of the lower order ones for a given quadrature point $\tilde \xi$. Therefore, we need to find the linear weights $d_j$ such that
%
\begin{equation}\label{eq:ideal_w_problem}
v^{ho}(\tilde \xi) = \sum_{j=0}^2 d_j \,v^{lo}_j(\tilde \xi) \quad\Longleftrightarrow\quad 
\sum_{\ell=-2}^{2} c^{ho}_{\ell}(\tilde \xi) \,u_{i+\ell} = \sum_{j=0}^2 \sum_{\ell=-j}^{2-j} d_j \, c^{lo}_{j\ell}(\tilde \xi) \,u_{i+\ell}, \quad \forall u_{i+\ell}.
\end{equation}
%
Since \eqref{eq:ideal_w_problem} must hold for any quintuplet $\lbrace u_{i+\ell} \rbrace _{\ell=-2}^{2}$, we can write a system of five equations in the 3 linear weights $d_j$ for each quadrature point $\tilde \xi$, i.e.,
%
\begin{equation}
%\begin{cases}
\sum_{j=0}^2 d_j \, c^{lo}_{j \ell}(\tilde \xi) = c^{ho}_{\ell}(\tilde \xi), \quad \forall \ell = -2,\dots,2. \\
%\end{cases}
\end{equation}
%
This is an overdetermined system with five equations and only three unknowns $d_j$ that can be easily solved by means of a least squares method. Moreover, the solutions found verify exactly all the equations, implying that some of the equations are linearly dependent.
%%
%\begin{equation}
%\underline{\underline{C}}^{lo}\,\underline{d} = \underline{\underline{C}}^{ho} \quad\Longrightarrow\quad 
%(\underline{\underline{C}}^{lo})^T \underline{\underline{C}}^{lo} \,\underline{d} = (\underline{\underline{C}}^{lo})^T \underline{\underline{C}}^{ho} \quad\Longrightarrow\quad
%\underline{d} = \left((\underline{\underline{C}}^{lo})^T \underline{\underline{C}}^{lo}\right)^{-1} (\underline{\underline{C}}^{lo})^T \underline{\underline{C}}^{ho}
%\end{equation}
%%








==> WENO5GP4.tex <==
\section{WENO recontruction ($r=3$) with four-point Gaussian quadrature rule}\label{sec:WENO5GP4}
%
The goal of this section is to present the fifth order WENO reconstruction with four-point Gaussian quadrature rule.
Up to our knowledge, there is no reference in literature that explicitly define linear weights and polynomial coefficients needed for this WENO reconstruction.
Reference~\cite{titarev2004finite} well described the fifth-order WENO5 with two-point Gaussian quadrature rule, which unfortunately does not
allow to go beyond fourth order. Instead, with the four-point Gaussian quadrature rule, one could reach even eighth order.\\ 
Let us consider a one-dimensional cell $[\xi_{\iin},\xi_{\iip}]$, we hereafter provide the expressions for 
%
\begin{equation}
q(\xi_{\iip}^-)\;,\;\; q(\xi_{\iin}^+)\;,\;\; q\left(\xi_i\pm\frac{\Delta\xi}{2}\sqrt{\frac{3}{7}+\frac{2}{7}\sqrt{\frac{6}{5}}}\right)\;,\;\;  q\left(\xi_i\pm\frac{\Delta\xi}{2}\sqrt{\frac{3}{7}-\frac{2}{7}\sqrt{\frac{6}{5}}}\right),
\end{equation}
which are used for the first sweep (first two terms corresponding to the two boundaries) and the second sweep (the last two terms corresponding to the 4 quadrature points).
%
For $r=3$ we have only three candidate stencil for the reconstruction
%
\begin{equation}
S_0 = (i,i+1,i+2)\;,\;\;\;S_1 = (i-1,i,i+1)\;,\;\;\;S_2 = (i-2,i-1,i).
\end{equation}
%
The corresponding smoothness indicators are given by:
%
\begin{align*}
\beta_0 &= \frac{13}{12} \left( q_i - 2q_{i+1} + q_{i+2}\right)^2 + \frac{1}{4} \left( 3q_i - 4q_{i+1} + q_{i+2} \right)^2,   \\ 
\beta_1 &= \frac{13}{12} \left( q_{i-1} - 2q_i + q_{i+1}\right)^2 + \frac{1}{4} \left( q_{i-1} - q_{i+1} \right)^2,   \\ 
\beta_2 &= \frac{13}{12} \left( q_{i-2} - 2q_{i-1} + q_i\right)^2 + \frac{1}{4} \left( q_{i-2} - 4q_{i-1} + 3q_i \right)^2.      
\end{align*}
%
The optimal weights $d_m$ for the left boundary extrapolated value $q_{\iip}^-$ at $\xip$ are 
%
\begin{equation}
d_0 = \frac{3}{10}  \;,\;\;\;   d_1 = \frac{3}{5}    \;,\;\;\;  d_2 = \frac{1}{10}
\end{equation}
%
and $q_{\iip}^-$ is given by
%
\begin{equation}
q_{\iip}^- = \frac{1}{6}\omega_0 \left(-q_{i+2} + 5q_{i+1} + 2q_i\right) + \frac{1}{6}\omega_1 \left(-q_{i-1} + 5q_{i} + 2q_{i+1}\right) + \frac{1}{6}\omega_2 \left(2q_{i-2} - 7q_{i-1} + 11q_i\right).
\end{equation}
%
The optimal weights $d_m$ for the right boundary extrapolated value $q_{\iin}^+$ at $\xin$ are 
%
\begin{equation}
d_0 = \frac{1}{10}  \;,\;\;\;   d_1 = \frac{3}{5}    \;,\;\;\;  d_2 = \frac{3}{10}
\end{equation}
%
and $q_{\iin}^+$ is given by
%
\begin{equation}
q_{\iin}^+ = \frac{1}{6}\omega_0 \left(2q_{i+2} - 7q_{i+1} + 11q_i\right) + \frac{1}{6}\omega_1 \left(-q_{i+1} + 5q_{i} + 2q_{i-1}\right) + \frac{1}{6}\omega_2 \left(-q_{i-2} + 5q_{i-1} + 2q_i\right).
\end{equation}
%
For the first Gaussian quadrature point $\xi_1^q = \xi_i - \frac{\Delta\xi}{2}\sqrt{\frac{3}{7}+\frac{2}{7}\sqrt{\frac{6}{5}}}$, 
the optimal weights are:
%
\begin{align}
\begin{aligned}
d_0 &= \frac{269\,\sqrt{42}\,\sqrt{2\,\sqrt{30}+15}}{50428}-\frac{1751\,\sqrt{35}\,\sqrt{2\,\sqrt{30}+15}}{504280}-\frac{411\,\sqrt{30}}{100856}+\frac{21855}{100856}, \\
d_1 &= \frac{411\,\sqrt{30}}{50428}+\frac{28573}{50428}, \\
d_2 &= \frac{1751\,\sqrt{35}\,\sqrt{2\,\sqrt{30}+15}}{504280}-\frac{269\,\sqrt{42}\,\sqrt{2\,\sqrt{30}+15}}{50428}-\frac{411\,\sqrt{30}}{100856}+\frac{21855}{100856}.
%d_0 = 0.1229074124899195  \;,\;\;\;   d_1 = 0.6112504900322486    \;,\;\;\;  d_2 = 0.2658420974778319
\end{aligned}
\end{align}
%
The reconstructed value can be computed from the three polynomials associated to each stencil:
%
{\tiny 
\begin{align*}
%\begin{aligned}
p_0(\xi_1^q) &= \left(\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{3\,\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{85}{84}\right) \,q_i + \left(-\frac{\sqrt{5}\,\sqrt{6}}{70}-\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}-\frac{1}{42}\right) \,q_{i+1} + \left(\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i+2} ,\\ 
p_1(\xi_1^q) &= \left(\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i-1} + \left(\frac{41}{42}-\frac{\sqrt{5}\,\sqrt{6}}{70}\right) \,q_{i} +  \left(\frac{\sqrt{5}\,\sqrt{6}}{140}-\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i+1}, \\ 
p_2(\xi_1^q) &= \left(\frac{\sqrt{5}\,\sqrt{6}}{140}-\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i-2} + \left(\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}-\frac{\sqrt{5}\,\sqrt{6}}{70}-\frac{1}{42}\right) \,q_{i-1} + \left(\frac{\sqrt{5}\,\sqrt{6}}{140}-\frac{3\,\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{85}{84}\right) \,q_{i}  .
%p_0 &=  1.6968800354220990 \,q_i     -0.9631919150471715 \,q_{i+1} +0.2663118796250726 \,q_{i+2} \\ 
%p_1 &=  0.2663118796250726 \,q_{i-1} +0.8979443965468811 \,q_{i}   -0.1642562761719537 \,q_{i+1} \\ 
%p_2 &= -0.1642562761719537 \,q_{i-2} +0.7590807081409336 \,q_{i-1} +0.4051755680310201 \,q_{i}  
%\end{aligned}
\end{align*}
}%
%
For the second Gaussian quadrature point $\xi_2^q = \xi_i - \frac{\Delta\xi}{2}\sqrt{\frac{3}{7}-\frac{2}{7}\sqrt{\frac{6}{5}}}$, 
the optimal weights are:
%
\begin{align}
\begin{aligned}
d_0 &= \frac{411\,\sqrt{30}}{100856}-\frac{269\,\sqrt{42}\,\sqrt{15-2\,\sqrt{30}}}{50428}-\frac{1751\,\sqrt{35}\,\sqrt{15-2\,\sqrt{30}}}{504280}+\frac{21855}{100856}, \\ 
d_1 &= \frac{28573}{50428}-\frac{411\,\sqrt{30}}{50428}, \\
d_2 &= \frac{1751\,\sqrt{35}\,\sqrt{15-2\,\sqrt{30}}}{504280}+\frac{269\,\sqrt{42}\,\sqrt{15-2\,\sqrt{30}}}{50428}+\frac{411\,\sqrt{30}}{100856}+\frac{21855}{100856}.
%d_0 = 0.3498666917141379  \;,\;\;\;   d_1 = 0.5219691498503563    \;,\;\;\;  d_2 = 0.128164158435505
\end{aligned}
\end{align}
%
The reconstructed value can be then computed from the three polynomials associated to the three stencil:
%
{\tiny 
\begin{align*}
%\begin{aligned}
p_0(\xi_2^q) &= \left(\frac{3\,\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{85}{84}\right) \,q_i     + \left(\frac{\sqrt{5}\,\sqrt{6}}{70}-\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}-\frac{1}{42}\right) \,q_{i+1} + \left(\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{1}{84}\right) \,q_{i+2}, \\ 
p_1(\xi_2^q) &= \left(\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{1}{84}\right) \,q_{i-1} + \left(\frac{\sqrt{5}\,\sqrt{6}}{70}+\frac{41}{42}\right) \,q_{i}   + \left(\frac{1}{84}-\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}\right) \,q_{i+1}, \\ 
p_2(\xi_2^q) &= \left(\frac{1}{84}-\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}\right) \,q_{i-2} + \left(\frac{\sqrt{5}\,\sqrt{6}}{70}+\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}-\frac{1}{42}\right) \,q_{i-1} + \left(\frac{85}{84}-\frac{3\,\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}\right) \,q_{i}  .
%p_0 &=  1.2277675047716066 \,q_i     -0.2855444877507849 \,q_{i+1} +0.0577769829791784 \,q_{i+2} \\ 
%p_1 &=  0.0577769829791784 \,q_{i-1} +1.0544365558340714 \,q_{i}   -0.1122135388132497 \,q_{i+1} \\ 
%p_2 &= -0.1122135388132497 \,q_{i-2} +0.3944175994189276 \,q_{i-1} +0.7177959393943222 \,q_{i}  
%\end{aligned}
\end{align*}
}%
%
For the third Gaussian quadrature point $\xi_3^q = \xi_i + \frac{\Delta\xi}{2}\sqrt{\frac{3}{7}-\frac{2}{7}\sqrt{\frac{6}{5}}}$, 
the optimal weights are:
%
\begin{align}
\begin{aligned}
d_0 &= \frac{1751\,\sqrt{35}\,\sqrt{15-2\,\sqrt{30}}}{504280}+\frac{269\,\sqrt{42}\,\sqrt{15-2\,\sqrt{30}}}{50428}+\frac{411\,\sqrt{30}}{100856}+\frac{21855}{100856}, \\
d_1 &= \frac{28573}{50428}-\frac{411\,\sqrt{30}}{50428}, \\
d_2 &= \frac{411\,\sqrt{30}}{100856}-\frac{269\,\sqrt{42}\,\sqrt{15-2\,\sqrt{30}}}{50428}-\frac{1751\,\sqrt{35}\,\sqrt{15-2\,\sqrt{30}}}{504280}+\frac{21855}{100856}.
%d_0 = 0.1281641584355059  \;,\;\;\;   d_1 = 0.5219691498503563    \;,\;\;\;  d_2 = 0.3498666917141379
\end{aligned}
\end{align}
%
The reconstructed value can be then computed from the three polynomials associated to the three stencil:
%
{\tiny
\begin{align*}
%\begin{aligned}
p_0 (\xi_3^q)&= \left(\frac{85}{84}-\frac{3\,\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}\right) \,q_i     + \left(\frac{\sqrt{5}\,\sqrt{6}}{70}+\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}-\frac{1}{42}\right)\,q_{i+1} + \left(\frac{1}{84}-\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}\right)\,q_{i+2}, \\ 
p_1(\xi_3^q) &= \left(\frac{1}{84}-\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}\right) \,q_{i-1} + \left(\frac{\sqrt{5}\,\sqrt{6}}{70}+\frac{41}{42}\right)\,q_{i}   + \left(\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{1}{84}\right)\,q_{i+1}, \\ 
p_2(\xi_3^q) &= \left(\frac{\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{1}{84}\right) \,q_{i-2} + \left(\frac{\sqrt{5}\,\sqrt{6}}{70}-\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}-\frac{1}{42}\right)\,q_{i-1} + \left(\frac{3\,\sqrt{\frac{3}{7}-\frac{2\,\sqrt{5}\,\sqrt{6}}{35}}}{4}-\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{85}{84}\right)\,q_{i}  .
%p_0 &=  0.7177959393943222 \,q_i     +0.3944175994189276 \,q_{i+1} -0.1122135388132497 \,q_{i+2} \\ 
%p_1 &= -0.1122135388132497 \,q_{i-1} +1.0544365558340714 \,q_{i}   +0.0577769829791784 \,q_{i+1} \\ 
%p_2 &=  0.0577769829791784 \,q_{i-2} -0.2855444877507849 \,q_{i-1} +1.2277675047716066 \,q_{i}  
%\end{aligned}
\end{align*}
}%
%
For the fourth Gaussian quadrature point $\xi_4^q = \xi_i + \frac{\Delta\xi}{2}\sqrt{\frac{3}{7}+\frac{2}{7}\sqrt{\frac{6}{5}}}$, 
the optimal weights are:
%
\begin{align}
\begin{aligned}
d_0 &= \frac{1751\,\sqrt{35}\,\sqrt{2\,\sqrt{30}+15}}{504280}-\frac{269\,\sqrt{42}\,\sqrt{2\,\sqrt{30}+15}}{50428}-\frac{411\,\sqrt{30}}{100856}+\frac{21855}{100856},  \\ 
d_1 &= \frac{411\,\sqrt{30}}{50428}+\frac{28573}{50428} , \\
d_2 &= \frac{269\,\sqrt{42}\,\sqrt{2\,\sqrt{30}+15}}{50428}-\frac{1751\,\sqrt{35}\,\sqrt{2\,\sqrt{30}+15}}{504280}-\frac{411\,\sqrt{30}}{100856}+\frac{21855}{100856}.
%d_0 = 0.2658420974778319  \;,\;\;\;   d_1 = 0.6112504900322486    \;,\;\;\;  d_2 = 0.1229074124899195
\end{aligned}
\end{align}
%
The reconstructed value can be then computed from the three polynomials associated to the three stencil:
%
{\tiny
\begin{align*}
%\begin{aligned}
p_0 (\xi_4^q)&= \left(\frac{\sqrt{5}\,\sqrt{6}}{140}-\frac{3\,\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{85}{84}\right) \,q_i     + \left(\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}-\frac{\sqrt{5}\,\sqrt{6}}{70}-\frac{1}{42}\right) \,q_{i+1} + \left(\frac{\sqrt{5}\,\sqrt{6}}{140}-\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i+2}, \\ 
p_1(\xi_4^q) &= \left(\frac{\sqrt{5}\,\sqrt{6}}{140}-\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i-1} + \left(\frac{41}{42}-\frac{\sqrt{5}\,\sqrt{6}}{70}\right) \,q_{i}   + \left(\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i+1} ,\\ 
p_2 (\xi_4^q)&= \left(\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{1}{84}\right) \,q_{i-2} + \left(-\frac{\sqrt{5}\,\sqrt{6}}{70}-\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}-\frac{1}{42}\right) \,q_{i-1} + \left(\frac{\sqrt{5}\,\sqrt{6}}{140}+\frac{3\,\sqrt{\frac{2\,\sqrt{5}\,\sqrt{6}}{35}+\frac{3}{7}}}{4}+\frac{85}{84}\right) \,q_{i}  .
%p_0 &=  0.4051755680310201 \,q_i     +0.75908070814093369 \,q_{i+1}-0.1642562761719537 \,q_{i+2} \\ 
%p_1 &= -0.1642562761719537 \,q_{i-1} +0.8979443965468811 \,q_{i}   +0.2663118796250726 \,q_{i+1} \\ 
%p_2 &=  0.2663118796250726 \,q_{i-2} -0.9631919150471715 \,q_{i-1} +1.6968800354220990 \,q_{i}  
%\end{aligned}
\end{align*}
}%
%
%\todo{I'm not sure the equation is correct. The reconstruction is done only in quadrature points and equation \eqref{eq:sum polynom} is general with $p_m(\xi)$.}
For all Gaussian quadrature points the solution in $\xi$ can be easily built by assembling 
the three polynomials.
%Philipp: I do not get wthe prboelm maybe we can chat this week about it ....
%

